Reconstructing Graphs from Connected Triples

We introduce a new model of indeterminacy in graphs: instead of specifying all the edges of the graph, the input contains all triples of vertices that form a connected subgraph. In general, different (labelled) graphs may have the same set of connected triples, making unique reconstruction of the original graph from the triples impossible. We identify some families of graphs (including triangle-free graphs) for which all graphs have a different set of connected triples. We also give algorithms that reconstruct a graph from a set of triples, and for testing if this reconstruction is unique. Finally, we study a possible extension of the model in which the subsets of size $k$ that induce a connected graph are given for larger (fixed) values of $k$.

==> Labelled reconstruction_ connectivity queries/figures/d8.tex <==
% \begin{tikzpicture}
% \def \n {8}
% \def \radius {.75cm}
% \def \margin {0} % margin in angles, depends on the radius
% \def \dotsize {.6}
% \foreach \s in {1,...,\n}
% {
%   \draw[-, >=latex] ({360/\n * (\s - 1)+\margin}:\radius) 
%     arc ({360/\n * (\s - 1)+\margin}:{360/\n * (\s)-\margin}:\radius);
% }
% \foreach \s in {1,...,\n}
% {
%     \node[draw, circle, fill = white, scale =\dotsize] (\s) at ({360/\n * (\s - 1)}:\radius){};
% }
% \node[draw, circle, fill = white, scale =\dotsize] (a) at (0:{2*\radius}){};
% \draw (a) to (1);
% \end{tikzpicture}

\begin{tikzpicture}
\def \n {5}
\def \radius {.75cm}
\def \outradius{1.5cm}
\def \margin {0} % margin in angles, depends on the radius
\def \dotsize {.6}
\node[draw, circle, fill = white, scale =\dotsize] (apex) at (0,0){};
\foreach \s in {1,...,\n}
{
    \node[draw, circle, fill = white, scale =\dotsize] (\s) at ({360/\n * (\s - 1)}:\radius){};
    \draw (\s) -- (apex);
    \coordinate (v\s) at  ({360/\n * (\s - 1)}:\outradius){};
}
\draw (1) -- (2) -- (3) -- (4) -- (5) -- (1);

\coordinate (w1) at  (15:\outradius){};
\coordinate (w2) at  (-15:\outradius){};

 
\draw (1) to [out = 30] (w1);
\draw (3) -- (v3);

\draw (w1) arc [start angle = 15, end angle = 144, radius = \outradius];

 % \draw (1) arc [start angle=0, end angle=144, radius=\radius];
\end{tikzpicture}


==> Labelled reconstruction_ connectivity queries/triangulated-planar.tex <==
\subsection{Reconstructing triangulated planar graphs}
\label{subsec:planar}
A \emph{triangulated planar graph}, also called a \emph{maximal planar graph}, is a planar graph where every face (including the outer face) is a triangle.
By definition triangulated planar graphs on more than three vertices are $3$-connected.
Note that chordal graphs (graphs in which every cycle of more than three vertices has a chord) are sometimes also called triangulated graphs, but this is not the meaning we use here. Every triangulated planar graph is chordal, but the reverse direction is trivially false.

To show that triangulated planar graphs on at least seven vertices can be uniquely reconstructed, 
we take a similar approach as in the proof of \cref{twoconnected}.
We argue that we can recognise all vertices of degree at least five with their neighbours in cyclic order in a graph that is known to be a $4$-connected triangulated planar graph on at least six vertices.
We then argue that we can reconstruct all graphs on at least six vertices that are known to be $4$-connected triangulated planar graphs.
Finally, we will use this result to show we can reconstruct every graph on at least seven vertices that is known to be triangulated and planar.
We begin with some easy observations.

For a connected graph $G$ we say a set of vertices $S \subset V(G)$ satisfying $\emptyset \neq S \neq V(G)$ is a \emph{separator} if $G \setminus S$ is disconnected.
A \emph{separating triangle} is a separator of cardinality three that induces a triangle.

\begin{observation}
    \label{obs:4conn}
    Every separator of cardinality 3 in a triangulated planar graph on at least five vertices is a separating triangle. 
\end{observation}
Indeed, by definition triangulated planar graphs do not have separators of size at most two.
Moreover, minimal separators of triangulated planar graphs must be cliques.
It is a consequence of Euler's formula (given below) that every triangulated planar graph on seven vertices contains a vertex of degree five.
We call the 4-regular planar graph on six vertices the octahedron (See \cref{fig:6-vertex-triangulated-cases} for a depiction).

\begin{theorem}[Euler's formula]\label{thm:euler}
    Let $G$ be a connected plane graph.
    Then $$n - e + f = 2$$ where $n,e,f$ are equal to the number of vertices, edges and faces of $G$, respectively. 
\end{theorem}
\begin{corollary}\label{corr:euler-degree5}
    Every triangulated planar graph with no vertex of degree at least five contains at most six vertices.
    Moreover, the octahedron is the unique triangulated planar graph on six vertices with no vertex of degree five. 
\end{corollary}

For $\ell \geq 4$, we call the graph obtain from a cycle of length $\ell$ by adding a new vertex $v$ and making it adjacent to every other vertex an \emph{$\ell$-wheel}. We call $v$ the \emph{centre} of the $\ell$-wheel. The cycle that does not contain $v$ is called the $C_\ell$ of the $\ell$-wheel.
We will show that for every vertex $v$ of degree $\ell \geq 5$ in a graph that is known to be triangulated, 4-connected, and planar the graph induced by $v$ and its neighbours is an $\ell$-wheel. For brevity, we will denote the set $N(v) \cup \{v\}$ as $N[v]$.

 \begin{lemma}\label{lem:nbd-of-degree-6}
    Suppose $G$ is a triangulated planar graph. Then for every $v \in V(G)$ of degree $\ell \geq 5$, the graph induced on $N[v]$ contains an $\ell$-wheel with centre $v$. Moreover, if $G$ is $4$-connected then the graph induced by $N[v]$ is an $\ell$-wheel.
 \end{lemma}
 \begin{proof}
    Let $v \in V(G)$ have degree at least five.
    Fix an embedding of $G$ and an orientation of the plane.
    Let $w_1, w_2, w_3, w_4, \dots, w_d$ be the neighbours of $v$ in cyclic order according to the embedding of $G[N(v)]$.
    Let $i \in \{1,2, \dots, d \}$.
    Then $w_i \dd v \dd w_{i+1}$ is a path bordering a face of $G$.
    Hence, there is some $w_iw_{i+1}$ path $P$ in $G \setminus v$ such that the union of $P$ and the path $w_i \dd v \dd w_{i+1}$ is a cycle bordering a face of $G$.
    Hence, since $G$ is triangulated $P$ must be a single edge.
    It follows that $w_1 \dd w_2 \dd w_3 \dd \dots \dd w_d \dd w_1$ is a cycle of $G$.
    This proves the first claim.

    
    Suppose $G$ is $4$-connected. 
     Suppose $w_iw_j$ is an edge for some non-consecutive $i,j \in \{1,2, \dots, d\}$ satisfying $i < j < d$.
    Since $G$ has no separating triangles there is a $w_{i+1}w_{j+1}$-path $Q$ in $G \setminus \{v,w_i, w_j\}$. But then $G[N[v]] \cup Q$ has a $K_5$ minor, a contradiction.
    Hence, $G[N[v]]$ is an $\ell$-wheel.
 \qed \end{proof}

%The $\ell$-fan is the graph obtained from a path of length $\ell$ by adding a new vertex adjacent to every other vertex.


\begin{observation}
    \label{obs:P5C5}
   For each $\ell \geq 5$, $C_\ell$ can be reconstructed.
\end{observation}

The result is trivial, but we include a proof for completeness.

\begin{proof}
Let $\ell \geq 5$ be an integer. We claim that $G$ is a $C_\ell$ with vertices $v_0, v_1, \dots, v_{\ell-1}$, in cyclic order if and only if the set of triples of $G$ is equal to ${X = \{v_iv_{i+1}v_{i+2} \ |}$ $ \ i= 1,2,\dots, \ell \}$ where indices are taken modulo $\ell$.

The \say{if} statement is trivial. 
Suppose $G$ is a graph on $\ell$ vertices $v_0, v_1, \dots, v_{\ell-1}$ and the $X$ is the set of triples of $G$.
Suppose $v_1v_2$ is not an edge of $G$. Then $v_0, v_3$ must be adjacent to both $v_1$ and $v_2$ since $v_0v_1v_2$ and $v_1v_2v_3$ are both triples of $G$. But then $v_0 \dd v_2 \dd v_3$ is a subgraph of $G$, a contradiction since $v_0v_2v_3 \not \in X$.
\qed \end{proof}

\begin{observation}\label{lem:apex}
A graph $G$ is an $\ell$-wheel if and only if there is some vertex $v$ that appears in $\binom{\ell}{2}$ triples and $G \setminus v$ is a $C_{\ell}$.
\end{observation}


% \begin{lemma}\label{lem:apex}
%     % We claim that $G$ is a $\ell$-wheel ($\ell$-fan) if and only if there is some vertex $v$ that appears in $\binom{\ell}{2}$ triples and $G \setminus v$ is a $C_{\ell}$ (resp. $P_{\ell}$).
%     We claim that $G$ is a $\ell$-wheel ($\ell$-fan) if and only if there is some vertex $v$ that appears in $\binom{\ell}{2}$ triples and $G \setminus v$ is a $C_{\ell}$ (resp. $P_{\ell}$).
% \end{lemma}
% \begin{proof}
%     Let $G$ be a graph on $\ell$ vertices.
%     Clearly, the lemma holds if $G$ is a $m$-wheel or if $G$ is a $m$-fan.
%     Suppose some $v \in V(G)$ appears in $\binom{\ell }{2}$ triples and $G \setminus v$ is a $C_{\ell}$ or $P_{\ell}$. Suppose $v$ is not adjacent to some $w \in G \setminus v$. Then since $vww'$ is a triple for each $w' \in G \setminus \{v, w\}$ it follows that $w$ has degree four in $G \setminus \{v\}$. But this is a contradiction since every vertex of $G \setminus v$ is an $\ell$-wheel or $\ell$-fan.
%     Hence $G$ is a $\ell$-fan if $G\setminus v$ is a $P_{\ell}$ and $G$ is a $\ell$-wheel if $G \setminus v$ is a $C_{\ell}$.    
% \qed \end{proof}
 By combining \cref{obs:P5C5} and \cref{lem:apex}, we obtain for each $\ell \geq 5$, we can reconstruct the $\ell$-wheel when we know the graph in question is triangulated, planar and $4$-connected. 
It follows from, \cref{obs:P5C5}, \cref{lem:apex} and \cref{lem:nbd-of-degree-6} that: 
\begin{corollary}
\label{corr:degree-five-vertex}
    If $G$ is known to be a triangulated planar graph without any separating triangles, for each $v \in G$ of degree at least five we can reconstruct the graph induced by $v$ and its neighbours.
\end{corollary}

\begin{lemma}\label{lem:reconstruct-4-conn-case-planar}
    Every connected graph $G$ on at least seven vertices that is known to be planar, triangulated and $4$-connected can be reconstructed. 
\end{lemma}
\begin{proof}
    It is an easy consequence of Euler's formula (given as \cref{corr:degree-five-vertex}), that $G$ must have a vertex $v$ of degree at least five.
    By \cref{corr:degree-five-vertex}, we can reconstruct the graph induced by $N[v]$ since $G$ is $4$-connected.
    We say the distance between two vertices $x,y$ is the number $d(x,y)$ of edges on a shortest path between them.
    Let $B_{m}(v)$ denote the graph induced by the set of vertices of distance at most $m$ from $v$.
    Suppose for some $\ell \geq 2$, we can reconstruct $B_{\ell-1}(v)$ from the connected triples of $G$.
    \begin{claim}
    We can determine the set of vertices $w \in N(x)$ that are of distance $\ell$ from $v$ for every vertex $x$ satisfying $d(v,x) = \ell-1$.\label{stmt:nbrlist}
    \end{claim}
    Since $\ell \geq 2$, there is an edge between $x$ and some vertex $y$ satisfying $d(v, y) = \ell -2$.
    Then, $q$ is a neighbour of $x$ of distance $\ell$ from $v$ if and only if $q \not \in V(B_{\ell -1}(v))$ and $qxy$ is a connected triple.
    Thus, we reconstruct the list of neighbours of $x$ of distance $\ell$ from $v$. This proves the claim.
    \\
    \\
    %Let $u$ be a neighbor of $x$ of distance $\ell$.
    For a vertex $b \in G$ and integer $m$ let $N^{m}_v(b)$ denote the set of neighbours of $b$ of distance at most $m$ from $v$.
    Then by the previous claim we can reconstruct the set $N^{\ell -1}_v(w)$ for each $w \in G$. Moreover, we can determine the set of vertices of distance $\ell$ from $v$. 
    Let $u$ be a vertex of distance $\ell$ from $v$.
    We complete the proof by showing we can reconstruct the set $N^\ell_v(u)$.
    Let $z \neq u$ be a vertex of distance $\ell$ from $v$.


    \begin{claim}
        Let $z$ be a vertex of distance $\ell$ from $v$.
        Suppose that $z$ and $u$ are adjacent. Then, if $z$ and $u$ have a common neighbour $x$ satisfying $d(v,x) = \ell -1$ it follows that $x$ must have degree at least five. Moreover, the edge $zu$ can be reconstructed.
    \end{claim}

    Since $\ell \geq 2$, by definition $x$ must have a neighbour $x'$ of distance $\ell -2$ from $v$. Then $z,u$ are both not adjacent to $x'$.
    Since $G$ is triangulated, it follows that $x', x, u$ do not all occur together on a cycle bounding a face and $x', x, z$ do not all occur together on a cycle bounding a face.
    Because $G$ is planar there is a single face $C$ of $G \setminus x$ that contains all neighbours of $x$.
    Let $P_u$ be the $x'u$-path of $C$ that does not contain $z$ and let $P_z$ be the $x'z$-path of $C$ that does not contain $u$.
    Then, since $G$ is triangulated $x$ must have a neighbour in the interior of both $P_u$ and $P_z$.
    Hence, $x$ has degree at least five.
    So by \cref{corr:degree-five-vertex}, $G[N[x]]$ and thus the edge $uz$ can be reconstructed. 
    This proves the claim.
    \\
    \\
    We complete the proof by showing that we can determine the edges from $u$ to vertices $z$ satisfying $d(v,z) = \ell$ and $N^{\ell-1}_v(z) \cap N^{\ell -1}_v(u) = \emptyset$.
    Let $x$ denote a neighbour of $u$ that is of distance $\ell-1$ from $v$.
    Then $z$ and $u$ are adjacent if and only if $xuz$ is a triple.
\qed \end{proof}


We can also recognise \say{small enough} separators of a graph. We only need this result for separators of size three on graphs with at least six vertices.

\begin{observation}
    \label{lem:recognising-separators}
    Let $G$ be a connected graph on $n$ vertices and let $S \subseteq V(G)$ have cardinality at most $n -3$.
    Then $S$ is a separator if and only if it is possible to partition $V(G) \setminus S$ into two non-empty parts $V_1, V_2$  such that any triple containing a vertex from $V_1$ and a vertex from $V_2$ must contain a vertex from $S$. 
\end{observation}
%\linda{I don't think we need to include this proof.}
% \begin{proof}
%     If \(S\) is a separator the observation is trivial. 
%     Conversely, if \(S\) is not a separator, the remainder of the graph must form one connected component.
%     If there are at least three remaining vertices, this means that, for any choice of \(V_1\) and \(V_2\), there must be a vertex \(x \in V_1\) with a neighbour \(y \in V_2\), and a third vertex \(z\) that neighbours \(x\) and/or \(y\).
%     We then have a triple containing vertices from \(V_1\) and \(V_2\) but not containing any element of \(S\).
% \qed \end{proof}

Using the fact that we can detect separators of size three, we will show that all triangulated planar graphs of at least seven vertices have a unique reconstruction by performing recursion along separating triangles.
We will need the following observation.

\begin{observation}\label{obs:defining-the-recursion}
Let $G$ be a triangulated plane graph and let $S$ be a separator of size three in $G$.
Then $G \setminus S$ has exactly two components $V_1, V_2$ and $G[S\cup V_1]$ and $G[S \cup V_2]$ are both triangulated planar graphs. 
\end{observation}

\cref{obs:defining-the-recursion} follows from the fact that if $G$ is a triangulated planar graph every component of $G \setminus S$ would need to have an edge to each vertex of $S$.
Since $S$ is the vertex set of a triangle by \cref{obs:4conn} and planar graphs do not have $K_{3,3}$ subgraphs it follows that there can be at most two components of $G \setminus S$.
We can use \cref{obs:defining-the-recursion} to perform recursion on $G[(V(H) \cup V_1]$ and $G[V(H) \cup V_2]$ until we are left with either a triangulated planar graph with no separating triangles with at least seven vertices (which we can handle by \cref{lem:reconstruct-4-conn-case-planar}) or a triangulated planar graph on at most six vertices.
Next, we will show that if we end up with a triangulated planar graph on at most six vertices from this procedure, we are able to reconstruct it.
We begin by describing the triangulated planar graphs on at most six vertices.

For $\ell \geq 3$, we call a graph obtained from an $\ell$-wheel by adding as many chords as possible to the $C_\ell$ while keeping the graph planar a \emph{triangulated $\ell$-wheel}.
Note when $\ell \leq 5$, this is uniquely defined, up to labelling (see \cref{fig:6-vertex-triangulated-cases}).
Moreover, any triangulated planar graph on $n$ vertices containing a vertex of degree $n-1$ must be a triangulated $(n-1)$-wheel.

\begin{figure}[t]
    \centering
    \includegraphics[width=.7\textwidth]{figures/base-case-planar.png}
    \caption{A depiction of all the distinct (unlabelled) triangulated planar graphs on five or six vertices. From left to right, the graphs are the triangulated 4-wheel, triangulated 5-wheel, and the octahedron.}
    %LC: If you want you can replace this figure with one more similar to the style of the other figures in this paper.
    %I chose this figure instead of the previous version of 6-vertex-triangulated-cases figure because the previous version was a bit confusing to me since it depicted 4 isomorphic graphs with really different planar embeddings and I think it is easier just to have one drawing and point out there are different cases depending on where the seperating triangle was
    \label{fig:6-vertex-triangulated-cases}
\end{figure}

\begin{observation}\label{obs:cases}
Every triangulated planar graph on at most six vertices is either a $K_3$, a $K_4$, a triangulated $4$-wheel, an octahedron or a triangulated $5$-wheel. 
\end{observation}

We are now ready to prove the base case of our recursion.

\begin{lemma}\label{lem:small-planar}
    Let $G$ be a graph on at least seven vertices that is known to be triangulated and planar.
    Suppose $G$ has a separator $S$ of size three and let $V_1$ be a component of $G \setminus S$ of size at most three.
    Then $G[S \cup V_1]$ can be reconstructed using the triples of $G$ and the knowledge of the labels of $S, V_1$ and the fact that $S$ is a separator of $G$.
\end{lemma}
\begin{proof}
    Let $G'$ denote the graph $G[S \cup V_1]$.
    Since $G \setminus V_1$ is non-empty and $G$ is a triangulated planar graph each vertex $s \in S$ must have a neighbour in $u_s \in G \setminus G'$.
    Then, we can determine the edges between $S$ and $V_1$ by checking if $su_sv$ is a triple for each $s \in S$ and $v \in V_1$.
    Hence, we need only show that we can reconstruct the edges between vertices of $V_1$.
    This is trivial when $G'$ has four vertices.
    When $G'$ has five vertices it must be 4-connected by \cref{obs:cases} so the two vertices in $V_1$ must be adjacent.
    
    When $G'$ has six vertices, it is either the octahedron or the triangulated 5-wheel.
    Every vertex in the octahedron has degree four and the triangulated 5-wheel has exactly two vertices of degree four.
    Thus, since we know the edges incident to $S$ in $G'$ we can determine whether $G'$ is an octahedron or a triangulated 5-wheel. Note that the graph obtained after removing the vertex set of any triangle in the octahedron is a triangle.
    Hence, $V_1$ must induce a triangle. So we can reconstruct $G'$ if it is an octahedron.

    We complete the proof by supposing $G'$ is a triangulated $5$-wheel and showing we can reconstruct $G'$. Note the triangulated $5$-wheel has exactly two vertices of degree 3, degree 4 and degree 5.
    Moreover, it has an isomorphism mapping the vertex of degree $i$ to the other vertex of degree $i$ for each $i \in \{3,4,5\}$.
    We say $S$ has degrees $(n_1,n_2,n_3)$ if the vertices of $S$ can be ordered so that the $i$-th vertex has degree $n_i$ in $G'$. %LC: rephrase to make less confusing?
    Because of the symmetry of $G'$, the unlabelled graph on $G' \setminus S$ is determined by the degrees of $S$.
    Since $S$ induces a triangle, there are only four possible degrees $S$ can have $(5, 5, 4)$, $(5,5,3)$, $(5,4,4)$, $(5,4,3)$.
    Moreover, since we already reconstructed the edges between $S$ and $G' \setminus S$, if there is some $x, y \in G' \setminus S$ such that $y$ has a neighbour $s \in S$ that is not adjacent to $x$ then we can test if $x$ and $y$ are adjacent by checking if $sxy$ is a triple.
    It is not difficult to see that these observations together are enough to reconstruct $G'$.
\qed \end{proof}

We are now ready to prove the main result of this subsection.
\repeattheorem{triangulated}
\begin{proof}
    Let $G$ be a triangulated planar graph on at least seven vertices.
    By \cref{lem:recognising-separators}, we can determine if $G$ has a separator of size $3$.
    If it doesn't, we can reconstruct $G$ by \cref{lem:reconstruct-4-conn-case-planar}. So, we may assume $G$ has a separator $S$ of size 3.
    Then $G \setminus S$ has exactly two components, and we can recognise their vertex sets $V_1, V_2$ by \cref{lem:recognising-separators} and \cref{obs:defining-the-recursion}.
    Moreover, by \cref{obs:defining-the-recursion} both $G[V_1 \cup S]$ and $G[V_2 \cup S]$ are planar and triangulated.
    For $i\in \{1,2\}$, if $G[V_i \cup S]$ contains at most six vertices we can reconstruct $G[V_i \cup S]$ by \cref{lem:small-planar}.
    Otherwise, we perform recursion on $G[V_i \cup S]$.
\qed \end{proof}

Note that, while our proof is constructive, it does not lead to a faster algorithm than the general cubic or \(O(n \cdot \norm{T})\) time algorithm described in \cref{sec:algorithm}.

==> figures/d8.tex <==
% \begin{tikzpicture}
% \def \n {8}
% \def \radius {.75cm}
% \def \margin {0} % margin in angles, depends on the radius
% \def \dotsize {.6}
% \foreach \s in {1,...,\n}
% {
%   \draw[-, >=latex] ({360/\n * (\s - 1)+\margin}:\radius) 
%     arc ({360/\n * (\s - 1)+\margin}:{360/\n * (\s)-\margin}:\radius);
% }
% \foreach \s in {1,...,\n}
% {
%     \node[draw, circle, fill = white, scale =\dotsize] (\s) at ({360/\n * (\s - 1)}:\radius){};
% }
% \node[draw, circle, fill = white, scale =\dotsize] (a) at (0:{2*\radius}){};
% \draw (a) to (1);
% \end{tikzpicture}

\begin{tikzpicture}
\def \n {5}
\def \radius {.75cm}
\def \outradius{1.5cm}
\def \margin {0} % margin in angles, depends on the radius
\def \dotsize {.6}
\node[draw, circle, fill = white, scale =\dotsize] (apex) at (0,0){};
\foreach \s in {1,...,\n}
{
    \node[draw, circle, fill = white, scale =\dotsize] (\s) at ({360/\n * (\s - 1)}:\radius){};
    \draw (\s) -- (apex);
    \coordinate (v\s) at  ({360/\n * (\s - 1)}:\outradius){};
}
\draw (1) -- (2) -- (3) -- (4) -- (5) -- (1);

\coordinate (w1) at  (15:\outradius){};
\coordinate (w2) at  (-15:\outradius){};

 
\draw (1) to [out = 30] (w1);
\draw (3) -- (v3);

\draw (w1) arc [start angle = 15, end angle = 144, radius = \outradius];

 % \draw (1) arc [start angle=0, end angle=144, radius=\radius];
\end{tikzpicture}

